A study of dust properties in the inner sub-au region of the Herbig Ae star HD 169142 with VLTI/PIONIER

An essential step to understanding protoplanetary evolution is the study of disks that contain gaps or inner holes. The pretransitional disk around the Herbig star HD 169142 exhibits multi-gap disk structure, differentiated gas and dust distribution, planet candidates, and near-infrared fading in the past decades, which make it a valuable target for a case study of disk evolution. Using near-infrared interferometric observations with VLTI/PIONIER, we aim to study the dust properties in the inner sub-au region of the disk in the years 2011-2013, when the object is already in its near-infrared faint state. We first performed simple geometric modeling to characterize the size and shape of the NIR-emitting region. We then performed Monte-Carlo radiative transfer simulations on grids of models and compared the model predictions with the interferometric and photometric observations. We find that the observations are consistent with optically thin gray dust lying at Rin ~ 0.07 au, passively heated to T ~ 1500 K. Models with sub-micron optically thin dust are excluded because such dust will be heated to much higher temperatures at similar distance. The observations can also be reproduced with a model consisting of optically thick dust at Rin ~ 0.06 au, but this model is plausible only if refractory dust species enduring ~2400 K exist in the inner disk.

==> fig/MCRT_1comp_Thick_fine_dataset1/AutomaticInfo.tex <==


\providecommand\TabulatedCodeForParameterSystem{}
\renewcommand\TabulatedCodeForParameterSystem{
$L_*~[L_\sun]$
  & \ParameterRange{4}{5}
  & $5$
  & $4.8$\\
$i~[\degree]$
  & $0$
  & $-$
  & $0$\\
$\mathrm{PA}~[\degree]$
  & $0$
  & $-$
  & $0$\\
}

\providecommand\TabulatedCodeForParameterInnerDisk{}
\renewcommand\TabulatedCodeForParameterInnerDisk{
$R_\mathrm{in}$ $[\AU]$
  & \ParameterRange{0.04}{0.2}
  & $12$
  & $0.062$\\
$W_\mathrm{ring}$
  & $0.5$
  & $-$
  & $0.5$\\
$h_\mathrm{in}$
  & \ParameterRange{0.01}{0.04}
  & $12$
  & $0.031$\\
$q$
  & $0$
  & $-$
  & $0$\\
$p$
  & $0$
  & $-$
  & $0$\\
$\tau$
  & $1000$
  & $-$
  & $1000$\\
$n$
  & $-3.5$
  & $-$
  & $-3.5$\\
$f_\mathrm{carbon}$
  & $0.5$
  & $-$
  & $0.5$\\
}

\providecommand\ModelNumber{}
\renewcommand\ModelNumber{$ 5{\times}12{\times}12 = 720 $
}

\providecommand\BestChiSquare{}
\renewcommand\BestChiSquare{1.29
}


==> fig/MCRT_1comp_Thick_fine_dataset1/ManualModelInfo.tex <==

\providecommand\TabulatedCodeForParameterOuterDisk{}
\renewcommand\TabulatedCodeForParameterOuterDisk{
$k$
& $0.13$
& $-$
& $0.13$
\\
}


==> fig/MCRT_1comp_Thin_dataset1/AutomaticInfo.tex <==


\providecommand\TabulatedCodeForParameterSystem{}
\renewcommand\TabulatedCodeForParameterSystem{
$L_*~[L_\sun]$
  & \ParameterRange{5.5}{4}
  & $4$
  & $4.5$\\
$i~[\degree]$
  & $0$
  & $-$
  & $0$\\
$\mathrm{PA}~[\degree]$
  & $0$
  & $-$
  & $0$\\
}

\providecommand\TabulatedCodeForParameterInnerDisk{}
\renewcommand\TabulatedCodeForParameterInnerDisk{
$R_\mathrm{in}$ $[\AU]$
  & \ParameterRange{0.04}{0.4}
  & $8$
  & $0.077$\\
$W_\mathrm{ring}$
  & $0.5$
  & $-$
  & $0.5$\\
$h_\mathrm{in}$
  & $0.6$
  & $-$
  & $0.6$\\
$q$
  & $0$
  & $-$
  & $0$\\
$p$
  & $0$
  & $-$
  & $0$\\
$\tau$
  & \ParameterRange{0.05}{0.3}
  & $7$
  & $0.091$\\
$n$
  & \ParameterRange{-5}{-2}
  & $7$
  & $-2.5$\\
$f_\mathrm{carbon}$
  & \ParameterRange{0}{1}
  & $3$
  & $1$\\
}

\providecommand\ModelNumber{}
\renewcommand\ModelNumber{$ 4{\times}8{\times}7{\times}3{\times}7 = 4704 $
}

\providecommand\BestChiSquare{}
\renewcommand\BestChiSquare{1.53
}


==> fig/MCRT_1comp_Thin_dataset1/ManualModelInfo.tex <==

\providecommand\TabulatedCodeForParameterOuterDisk{}
\renewcommand\TabulatedCodeForParameterOuterDisk{
$k$
& $0.13$
& $-$
& $0.13$
\\
}


==> fig/MCRT_1comp_Thin_fine_dataset1/AutomaticInfo.tex <==


\providecommand\TabulatedCodeForParameterSystem{}
\renewcommand\TabulatedCodeForParameterSystem{
$L_*~[L_\sun]$
  & \ParameterRange{4}{5}
  & $5$
  & $4.8$\\
$i~[\degree]$
  & $0$
  & $-$
  & $0$\\
$\mathrm{PA}~[\degree]$
  & $0$
  & $-$
  & $0$\\
}

\providecommand\TabulatedCodeForParameterInnerDisk{}
\renewcommand\TabulatedCodeForParameterInnerDisk{
$R_\mathrm{in}$ $[\AU]$
  & \ParameterRange{0.04}{0.2}
  & $12$
  & $0.072$\\
$W_\mathrm{ring}$
  & $0.5$
  & $-$
  & $0.5$\\
$h_\mathrm{in}$
  & $0.6$
  & $-$
  & $0.6$\\
$q$
  & $0$
  & $-$
  & $0$\\
$p$
  & $0$
  & $-$
  & $0$\\
$\tau$
  & \ParameterRange{0.05}{0.2}
  & $12$
  & $0.083$\\
$n$
  & \ParameterRange{-3.5}{-2}
  & $4$
  & $-2$\\
$f_\mathrm{carbon}$
  & $0.5$
  & $-$
  & $0.5$\\
}

\providecommand\ModelNumber{}
\renewcommand\ModelNumber{$ 5{\times}12{\times}12{\times}4 = 2880 $
}

\providecommand\BestChiSquare{}
\renewcommand\BestChiSquare{1.36
}


==> fig/MCRT_1comp_Thin_fine_dataset1/ManualModelInfo.tex <==

\providecommand\TabulatedCodeForParameterOuterDisk{}
\renewcommand\TabulatedCodeForParameterOuterDisk{
$k$
& $0.13$
& $-$
& $0.13$
\\
}


==> fig/MCRT_1comp_Thin_scanW_dataset1/AutomaticInfo.tex <==


\providecommand\TabulatedCodeForParameterSystem{}
\renewcommand\TabulatedCodeForParameterSystem{
$L_*~[L_\sun]$
  & $4.8$
  & $-$
  & $4.8$\\
$i~[\degree]$
  & $0$
  & $-$
  & $0$\\
$\mathrm{PA}~[\degree]$
  & $0$
  & $-$
  & $0$\\
}

\providecommand\TabulatedCodeForParameterInnerDisk{}
\renewcommand\TabulatedCodeForParameterInnerDisk{
$R_\mathrm{in}$ $[\AU]$
  & \ParameterRange{0.02}{0.2}
  & $21$
  & $0.045$\\
$W_\mathrm{ring}$
  & \ParameterRange{0.2}{5}
  & $6$
  & $3$\\
$h_\mathrm{in}$
  & $0.6$
  & $-$
  & $0.6$\\
$q$
  & $0$
  & $-$
  & $0$\\
$p$
  & $0$
  & $-$
  & $0$\\
$\tau$
  & $0.083$
  & $-$
  & $0.083$\\
$n$
  & \ParameterRange{-5}{-2}
  & $7$
  & $-2$\\
$f_\mathrm{carbon}$
  & $0.5$
  & $-$
  & $0.5$\\
}

\providecommand\ModelNumber{}
\renewcommand\ModelNumber{$ 21{\times}6{\times}7 = 882 $
}

\providecommand\BestChiSquare{}
\renewcommand\BestChiSquare{1.32
}


==> fig/MCRT_1comp_Thin_scanW_dataset1/ManualModelInfo.tex <==

\providecommand\TabulatedCodeForParameterOuterDisk{}
\renewcommand\TabulatedCodeForParameterOuterDisk{
$k$
& $0.13$
& $-$
& $0.13$
\\
}

